Localization in Unstructured Environments: Towards Autonomous Robots in Forests with Delaunay Triangulation

Autonomous harvesting and transportation is a long-term goal of the forest industry. One of the main challenges is the accurate localization of both vehicles and trees in a forest. Forests are unstructured environments where it is difficult to find a group of significant landmarks for current fast feature-based place recognition algorithms. This paper proposes a novel approach where local observations are matched to a general tree map using the Delaunay triangularization as the representation format. Instead of point cloud based matching methods, we utilize a topology-based method. First, tree trunk positions are registered at a prior run done by a forest harvester. Second, the resulting map is Delaunay triangularized. Third, a local submap of the autonomous robot is registered, triangularized and matched using triangular similarity maximization to estimate the position of the robot. We test our method on a dataset accumulated from a forestry site at Lieksa, Finland. A total length of 2100\,m of harvester path was recorded by an industrial harvester with a 3D laser scanner and a geolocation unit fixed to the frame. Our experiments show a 12\,cm s.t.d. in the location accuracy and with real-time data processing for speeds not exceeding 0.5\,m/s. The accuracy and speed limit is realistic during forest operations.

==> pics/6_trunks_observed_plot.tex <==
% This file was created by tikzplotlib v0.8.5.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color1}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color2}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color3}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis background/.style={fill=white},%99!black},
    axis line style={white},
    legend cell align={left},
    % legend style={at={(0.97,0.03)}, anchor=south east, draw=white!80.0!black},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xlabel={Frames},
    xmajorgrids,
    xmin=-34.95, xmax=733.95,
    xtick style={color=lightgray},
    y grid style={fill=white!96!black},
    ylabel={Number of trunks Observed},
    ymajorgrids,
    ymin=-0.450000000000001, ymax=202,
    ytick style={color=lightgray}
]
\addplot [thin, color0, mark=*, mark size=0.42, mark options={solid}]
table {%
1 25
2 28
3 23
4 25
5 27
6 26
7 28
8 26
9 30
10 24
11 21
12 24
13 23
14 21
15 19
16 15
17 19
18 21
19 26
20 26
21 22
22 23
23 20
24 13
25 27
26 19
27 22
28 21
29 19
30 28
31 29
32 16
33 19
34 21
35 23
36 20
37 8
38 22
39 12
40 15
41 15
42 23
43 19
44 22
45 20
46 20
47 21
48 18
49 24
50 26
51 36
52 35
53 32
54 26
55 23
56 20
57 17
58 16
59 23
60 18
61 11
62 16
63 23
64 25
65 18
66 16
67 21
68 15
69 23
70 25
71 32
72 34
73 39
74 27
75 29
76 29
77 34
78 25
79 40
80 27
81 27
82 34
83 30
84 29
85 28
86 39
87 30
88 29
89 41
90 33
91 34
92 37
93 31
94 46
95 34
96 33
97 37
98 41
99 37
100 31
101 32
102 37
103 42
104 45
105 43
106 39
107 44
108 42
109 44
110 39
111 33
112 44
113 47
114 46
115 42
116 51
117 60
118 53
119 54
120 65
121 64
122 46
123 46
124 10
125 38
126 43
127 33
128 26
129 33
130 35
131 38
132 23
133 36
134 36
135 41
136 49
137 47
138 38
139 49
140 53
141 52
142 48
143 64
144 58
145 56
146 55
147 53
148 54
149 60
150 60
151 57
152 53
153 54
154 52
155 56
156 48
157 43
158 47
159 54
160 49
161 42
162 58
163 50
164 52
165 53
166 62
167 60
168 46
169 50
170 55
171 60
172 60
173 53
174 51
175 50
176 63
177 59
178 61
179 56
180 64
181 44
182 39
183 42
184 53
185 47
186 57
187 58
188 49
189 54
190 50
191 56
192 55
193 52
194 52
195 54
196 62
197 59
198 61
199 72
200 64
201 75
202 62
203 55
204 58
205 61
206 47
207 58
208 69
209 72
210 59
211 57
212 63
213 53
214 44
215 39
216 51
217 42
218 50
219 56
220 52
221 62
222 58
223 67
224 63
225 64
226 63
227 68
228 63
229 62
230 77
231 65
232 62
233 62
234 60
235 66
236 71
237 66
238 58
239 69
240 63
241 58
242 54
243 56
244 58
245 53
246 62
247 52
248 47
249 51
250 52
251 53
252 49
253 66
254 65
255 72
256 56
257 59
258 58
259 61
260 28
261 55
262 61
263 58
264 67
265 68
266 61
267 61
268 48
269 63
270 57
271 53
272 49
273 57
274 65
275 54
276 54
277 63
278 54
279 60
280 67
281 61
282 58
283 70
284 60
285 68
286 79
287 57
288 47
289 59
290 59
291 63
292 54
293 60
294 64
295 56
296 66
297 51
298 58
299 47
300 49
301 60
302 61
303 65
304 57
305 55
306 56
307 69
308 54
309 57
310 58
311 65
312 55
313 59
314 60
315 64
316 57
317 57
318 57
319 63
320 61
321 60
322 56
323 50
324 50
325 53
326 53
327 53
328 59
329 58
330 63
331 67
332 61
333 48
334 58
335 60
336 57
337 59
338 52
339 48
340 56
341 55
342 56
343 53
344 53
345 49
346 58
347 61
348 52
349 59
350 59
351 59
352 57
353 64
354 64
355 58
356 62
357 57
358 60
359 60
360 58
361 52
362 63
363 66
364 64
365 59
366 59
367 54
368 56
369 60
370 62
371 70
372 61
373 74
374 72
375 77
376 69
377 87
378 75
379 64
380 59
381 65
382 66
383 71
384 67
385 52
386 51
387 59
388 66
389 71
390 66
391 66
392 69
393 64
394 69
395 65
396 66
397 65
398 70
399 69
400 70
401 76
402 70
403 61
404 64
405 62
406 61
407 65
408 68
409 72
410 67
411 67
412 61
413 64
414 64
415 58
416 60
417 66
418 60
419 60
420 59
421 70
422 57
423 67
424 67
425 61
426 64
427 64
428 63
429 80
430 80
431 76
432 39
433 72
434 75
435 64
436 59
437 60
438 57
439 64
440 63
441 56
442 63
443 67
444 71
445 62
446 65
447 58
448 67
449 64
450 64
451 66
452 55
453 60
454 67
455 67
456 60
457 72
458 72
459 73
460 69
461 74
462 71
463 73
464 68
465 61
466 60
467 58
468 51
469 62
470 58
471 56
472 60
473 59
474 61
475 61
476 60
477 57
478 62
479 64
480 66
481 59
482 72
483 70
484 70
485 63
486 62
487 66
488 65
489 63
490 63
491 68
492 70
493 50
494 65
495 55
496 63
497 59
498 57
499 62
500 61
501 57
502 61
503 58
504 54
505 61
506 65
507 52
508 60
509 61
510 63
511 58
512 70
513 68
514 63
515 61
516 57
517 62
518 53
519 67
520 63
521 62
522 68
523 58
524 66
525 72
526 68
527 59
528 58
529 55
530 63
531 69
532 66
533 56
534 52
535 51
536 55
537 73
538 69
539 52
540 52
541 66
542 67
543 69
544 60
545 59
546 57
547 59
548 63
549 62
550 63
551 67
552 53
553 65
554 61
555 68
556 63
557 58
558 67
559 68
560 66
561 64
562 64
563 69
564 73
565 69
566 61
567 60
568 59
569 57
570 64
571 67
572 66
573 65
574 58
575 60
576 57
577 63
578 61
579 63
580 51
581 65
582 55
583 47
584 63
585 68
586 56
587 53
588 56
589 56
590 55
591 58
592 51
593 54
594 52
595 59
596 57
597 66
598 67
599 67
600 66
601 64
602 70
603 67
604 79
605 63
606 63
607 63
608 61
609 69
610 74
611 72
612 61
613 66
614 57
615 61
616 72
617 51
618 63
619 60
620 59
621 47
622 54
623 67
624 60
625 57
626 61
627 51
628 61
629 68
630 65
631 70
632 70
633 77
634 73
635 70
636 66
637 53
638 55
639 59
640 65
641 68
642 61
643 70
644 67
645 74
646 81
647 69
648 70
649 67
650 80
651 63
652 54
653 49
654 61
655 56
656 54
657 53
658 56
659 47
660 48
661 47
662 47
663 48
664 49
665 56
666 52
667 56
668 58
669 50
670 51
671 55
672 52
673 47
674 54
675 48
676 51
677 53
678 48
679 44
680 58
681 47
682 46
683 59
684 53
685 56
686 53
687 50
688 48
689 50
690 56
691 61
692 62
693 64
694 69
695 63
696 55
697 47
698 55
699 64
};
\addlegendentry{1 frame}
\addplot [thin, color1, mark=triangle*, mark size=0.42, mark options={solid}]
table {%
3 90
6 88
9 89
12 83
15 87
18 88
21 88
24 84
27 87
30 92
33 75
36 78
39 78
42 79
45 80
48 92
51 101
54 93
57 69
60 71
63 88
66 83
69 93
72 105
75 93
78 89
81 113
84 106
87 102
90 125
93 117
96 102
99 92
102 104
105 106
108 111
111 112
114 122
117 135
120 146
123 94
126 93
129 100
132 87
135 110
138 133
141 133
144 144
147 142
150 132
153 132
156 104
159 126
162 129
165 131
168 130
171 125
174 117
177 151
180 136
183 110
186 132
189 137
192 131
195 146
198 135
201 142
204 118
207 144
210 137
213 115
216 115
219 139
222 135
225 147
228 140
231 135
234 144
237 137
240 140
243 136
246 115
249 115
252 141
255 132
258 127
261 143
264 148
267 137
270 128
273 148
276 134
279 147
282 144
285 152
288 124
291 132
294 137
297 115
300 131
303 132
306 138
309 146
312 140
315 136
318 134
321 136
324 115
327 126
330 135
333 108
336 133
339 141
342 115
345 126
348 144
351 148
354 137
357 118
360 134
363 127
366 118
369 130
372 127
375 147
378 125
381 134
384 126
387 122
390 133
393 135
396 135
399 133
402 130
405 136
408 121
411 135
414 138
417 130
420 133
423 135
426 138
429 160
432 130
435 138
438 123
441 140
444 129
447 121
450 129
453 130
456 142
459 141
462 129
465 129
468 125
471 123
474 124
477 135
480 134
483 141
486 134
489 136
492 131
495 124
498 120
501 117
504 133
507 119
510 128
513 123
516 129
519 136
522 143
525 144
528 126
531 134
534 120
537 125
540 134
543 127
546 134
549 119
552 137
555 129
558 140
561 134
564 140
567 117
570 123
573 125
576 123
579 123
582 123
585 118
588 124
591 122
594 114
597 145
600 146
603 126
606 134
609 132
612 120
615 128
618 125
621 125
624 124
627 135
630 135
633 127
636 111
639 128
642 130
645 143
648 134
651 124
654 117
657 107
660 103
663 97
666 94
669 104
672 95
675 108
678 112
681 117
684 107
687 109
690 118
693 129
696 112
};
\addlegendentry{3 frames}
\addplot [thin, color2, mark=square*, mark size=0.42, mark options={solid}]
table {%
0 91
5 111
10 100
15 97
20 95
25 101
30 97
35 85
40 99
45 108
50 113
55 87
60 89
65 96
70 114
75 111
80 128
85 124
90 137
95 108
100 116
105 126
110 134
115 143
120 145
125 108
130 104
135 128
140 159
145 153
150 143
155 130
160 141
165 144
170 140
175 153
180 151
185 139
190 164
195 163
200 154
205 153
210 149
215 136
220 165
225 165
230 177
235 156
240 173
245 141
250 158
255 153
260 156
265 146
270 153
275 171
280 170
285 168
290 155
295 141
300 149
305 155
310 171
315 165
320 146
325 145
330 141
335 139
340 143
345 146
350 169
355 139
360 147
365 144
370 156
375 154
380 157
385 137
390 167
395 149
400 144
405 140
410 162
415 145
420 166
425 155
430 151
435 149
440 155
445 143
450 155
455 165
460 159
465 144
470 137
475 147
480 161
485 155
490 144
495 137
500 134
505 141
510 139
515 156
520 155
525 143
530 155
535 126
540 150
545 154
550 159
555 157
560 152
565 139
570 139
575 141
580 135
585 140
590 133
595 145
600 156
605 150
610 136
615 143
620 141
625 136
630 142
635 130
640 147
645 139
650 135
655 114
660 108
665 100
670 103
675 113
680 118
685 129
690 132
695 123
};
\addlegendentry{5 frames}
\addplot [thin, color3, mark=pentagon*, mark size=0.42, mark options={solid}]
table {%
0 99
10 92
20 100
30 89
40 101
50 99
60 87
70 102
80 135
90 125
100 107
110 144
120 131
130 111
140 152
150 135
160 145
170 139
180 129
190 170
200 155
210 141
220 153
230 157
240 163
250 162
260 143
270 167
280 177
290 149
300 159
310 155
320 156
330 117
340 140
350 158
360 149
370 153
380 144
390 143
400 137
410 161
420 171
430 145
440 143
450 149
460 149
470 117
480 145
490 127
500 134
510 125
520 151
530 134
540 136
550 147
560 136
570 145
580 114
590 115
600 124
610 139
620 123
630 135
640 132
650 115
660 91
670 87
680 104
690 113
};
\addlegendentry{10 frames}
\end{axis}

\end{tikzpicture}


==> pics/7_feature_hit_plot.tex <==
% This file was created by tikzplotlib v0.8.5.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color1}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color2}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color3}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{axis}[
    height=\figureheight,
    width=\figurewidth,
    axis background/.style={fill=white},%!96!black},
    axis line style={white},
    legend cell align={left},
    legend style={draw=white!80.0!black},
    % legend style={at={(0.03,0.97)}, anchor=south east, draw=white!80.0!black},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xlabel={Frames},
    xmajorgrids,
    xmin=-33.9, xmax=733.9,
    xtick style={color=lightgray},
    y grid style={fill=white!96!black},
    ylabel={Number of features matched},
    ymajorgrids,
    ymin=-2.15, ymax=45.15,
    ytick style={color=black}
]
\addplot [thin, color0, mark=*, mark size=0.42, mark options={solid}]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
16 0
17 0
18 0
19 0
20 0
21 0
22 0
23 0
24 0
25 0
26 0
27 0
28 0
29 0
30 0
31 0
32 0
33 0
34 0
35 0
36 0
37 0
38 0
39 0
40 0
41 0
42 0
43 0
44 0
45 0
46 0
47 0
48 0
49 0
50 0
51 0
52 1
53 0
54 0
55 0
56 0
57 0
58 0
59 0
60 0
61 0
62 0
63 0
64 0
65 0
66 0
67 0
68 0
69 0
70 0
71 0
72 0
73 0
74 0
75 0
76 0
77 0
78 0
79 2
80 0
81 0
82 1
83 0
84 0
85 0
86 0
87 0
88 0
89 3
90 0
91 0
92 0
93 0
94 0
95 0
96 0
97 0
98 0
99 0
100 0
101 0
102 0
103 0
104 0
105 0
106 0
107 0
108 0
109 0
110 0
111 0
112 0
113 0
114 0
115 0
116 0
117 0
118 0
119 0
120 1
121 0
122 0
123 0
124 0
125 0
126 0
127 0
128 0
129 0
130 0
131 0
132 0
133 1
134 0
135 1
136 1
137 0
138 0
139 0
140 0
141 0
142 0
143 1
144 0
145 1
146 2
147 3
148 0
149 0
150 0
151 0
152 0
153 0
154 3
155 0
156 0
157 0
158 0
159 0
160 0
161 0
162 0
163 0
164 2
165 0
166 3
167 0
168 0
169 0
170 2
171 1
172 1
173 0
174 0
175 0
176 0
177 0
178 1
179 1
180 0
181 0
182 0
183 0
184 0
185 0
186 0
187 2
188 0
189 0
190 0
191 0
192 0
193 1
194 0
195 1
196 0
197 0
198 0
199 0
200 0
201 4
202 1
203 1
204 0
205 0
206 0
207 0
208 2
209 0
210 0
211 0
212 0
213 0
214 3
215 0
216 2
217 0
218 1
219 0
220 0
221 0
222 0
223 0
224 0
225 0
226 0
227 0
228 0
229 0
230 0
231 0
232 0
233 0
234 0
235 1
236 0
237 0
238 0
239 0
240 0
241 1
242 0
243 0
244 0
245 1
246 1
247 0
248 0
249 0
250 0
251 0
252 0
253 1
254 0
255 0
256 0
257 0
258 0
259 0
260 0
261 0
262 0
263 0
264 0
265 0
266 0
267 0
268 0
269 0
270 0
271 0
272 0
273 0
274 0
275 0
276 1
277 0
278 0
279 0
280 0
281 0
282 0
283 0
284 0
285 0
286 0
287 0
288 0
289 0
290 0
291 2
292 0
293 0
294 0
295 0
296 0
297 0
298 1
299 0
300 2
301 0
302 0
303 0
304 0
305 0
306 0
307 1
308 0
309 0
310 0
311 0
312 0
313 0
314 0
315 0
316 0
317 0
318 0
319 0
320 0
321 0
322 0
323 0
324 0
325 1
326 0
327 0
328 0
329 0
330 0
331 0
332 0
333 0
334 0
335 0
336 0
337 0
338 0
339 0
340 0
341 0
342 0
343 0
344 1
345 1
346 0
347 0
348 0
349 1
350 0
351 0
352 0
353 0
354 0
355 0
356 0
357 0
358 0
359 0
360 0
361 0
362 0
363 0
364 0
365 4
366 1
367 2
368 1
369 1
370 0
371 0
372 1
373 1
374 0
375 0
376 0
377 0
378 1
379 0
380 0
381 0
382 1
383 0
384 0
385 0
386 1
387 1
388 1
389 1
390 0
391 0
392 1
393 4
394 0
395 0
396 1
397 3
398 6
399 2
400 0
401 2
402 0
403 3
404 1
405 1
406 1
407 1
408 2
409 1
410 1
411 1
412 2
413 1
414 3
415 2
416 1
417 0
418 0
419 0
420 0
421 0
422 0
423 0
424 0
425 0
426 0
427 0
428 1
429 2
430 3
431 1
432 0
433 0
434 1
435 0
436 0
437 0
438 0
439 0
440 0
441 0
442 0
443 0
444 0
445 0
446 0
447 0
448 3
449 0
450 0
451 0
452 0
453 0
454 1
455 0
456 0
457 0
458 0
459 0
460 0
461 0
462 0
463 0
464 1
465 0
466 0
467 0
468 0
469 0
470 0
471 0
472 0
473 0
474 0
475 0
476 0
477 0
478 0
479 0
480 0
481 0
482 0
483 0
484 0
485 0
486 0
487 0
488 0
489 0
490 0
491 0
492 0
493 0
494 2
495 0
496 1
497 1
498 1
499 0
500 1
501 0
502 0
503 0
504 0
505 0
506 0
507 0
508 0
509 0
510 1
511 3
512 0
513 0
514 3
515 0
516 2
517 2
518 0
519 1
520 0
521 0
522 0
523 0
524 0
525 0
526 0
527 0
528 0
529 1
530 1
531 0
532 0
533 0
534 0
535 1
536 0
537 0
538 0
539 0
540 0
541 1
542 1
543 0
544 0
545 0
546 0
547 1
548 0
549 3
550 0
551 2
552 0
553 0
554 0
555 0
556 0
557 0
558 0
559 0
560 0
561 0
562 1
563 0
564 0
565 0
566 0
567 0
568 0
569 0
570 1
571 0
572 0
573 1
574 0
575 0
576 0
577 0
578 0
579 1
580 0
581 0
582 0
583 1
584 0
585 0
586 0
587 0
588 0
589 0
590 1
591 0
592 0
593 0
594 0
595 0
596 0
597 0
598 0
599 1
600 0
601 4
602 1
603 2
604 0
605 0
606 0
607 0
608 0
609 2
610 4
611 1
612 1
613 1
614 2
615 0
616 2
617 0
618 0
619 0
620 0
621 0
622 0
623 0
624 0
625 1
626 0
627 0
628 0
629 1
630 2
631 1
632 3
633 6
634 5
635 0
636 1
637 0
638 2
639 2
640 3
641 1
642 0
643 0
644 0
645 1
646 1
647 0
648 2
649 1
650 1
651 0
652 0
653 0
654 0
655 0
656 0
657 1
658 2
659 0
660 1
661 0
662 0
663 0
664 1
665 3
666 3
667 4
668 0
669 0
670 0
671 3
672 3
673 0
674 0
675 3
676 1
677 4
678 0
679 0
680 0
681 3
682 0
683 1
684 0
685 2
686 0
687 0
688 0
689 0
690 1
691 3
692 1
693 0
694 5
695 1
696 1
697 0
698 0
699 0
};
\addlegendentry{1 frame}
\addplot [thin, color1, mark=triangle*, mark size=0.42, mark options={solid}]
table {%
3 12
6 8
9 4
12 6
15 9
18 12
21 6
24 7
27 3
30 1
33 4
36 0
39 11
42 0
45 9
48 11
51 18
54 6
57 1
60 3
63 6
66 5
69 7
72 6
75 4
78 7
81 14
84 2
87 11
90 7
93 7
96 9
99 1
102 13
105 3
108 2
111 0
114 9
117 17
120 17
123 0
126 7
129 6
132 8
135 7
138 10
141 6
144 4
147 10
150 0
153 5
156 4
159 2
162 11
165 7
168 8
171 5
174 4
177 4
180 6
183 3
186 2
189 2
192 10
195 3
198 7
201 5
204 3
207 4
210 0
213 3
216 3
219 1
222 5
225 3
228 3
231 2
234 3
237 6
240 5
243 2
246 6
249 0
252 9
255 1
258 1
261 5
264 6
267 0
270 2
273 6
276 6
279 2
282 5
285 5
288 0
291 3
294 3
297 2
300 3
303 2
306 0
309 3
312 0
315 0
318 1
321 2
324 2
327 2
330 0
333 0
336 1
339 5
342 10
345 2
348 4
351 3
354 0
357 4
360 2
363 4
366 4
369 6
372 3
375 6
378 10
381 3
384 7
387 14
390 6
393 2
396 2
399 4
402 3
405 3
408 1
411 3
414 1
417 1
420 0
423 0
426 6
429 19
432 7
435 0
438 4
441 0
444 2
447 1
450 0
453 0
456 3
459 7
462 5
465 4
468 5
471 1
474 1
477 0
480 2
483 3
486 2
489 3
492 2
495 8
498 4
501 2
504 2
507 0
510 4
513 2
516 1
519 3
522 2
525 8
528 2
531 8
534 1
537 2
540 3
543 6
546 5
549 5
552 1
555 3
558 4
561 1
564 0
567 1
570 5
573 1
576 7
579 5
582 1
585 2
588 2
591 5
594 2
597 2
600 7
603 2
606 3
609 10
612 14
615 4
618 0
621 1
624 1
627 2
630 13
633 20
636 11
639 14
642 9
645 4
648 4
651 0
654 4
657 5
660 2
663 4
666 6
669 1
672 4
675 4
678 1
681 2
684 4
687 7
690 10
693 4
696 2
};
\addlegendentry{3 frames}
\addplot [thin, color2, mark=square*, mark size=0.42, mark options={solid}]
table {%
5 27
10 15
15 14
20 15
25 13
30 1
35 5
40 15
45 20
50 20
55 8
60 8
65 7
70 10
75 6
80 10
85 16
90 9
95 11
100 9
105 10
110 2
115 43
120 21
125 14
130 8
135 10
140 28
145 29
150 4
155 15
160 9
165 12
170 9
175 10
180 0
185 4
190 7
195 19
200 10
205 10
210 2
215 5
220 15
225 9
230 6
235 11
240 12
245 9
250 13
255 14
260 15
265 9
270 7
275 15
280 15
285 9
290 9
295 8
300 10
305 6
310 9
315 3
320 1
325 5
330 1
335 2
340 13
345 18
350 2
355 4
360 5
365 15
370 15
375 12
380 8
385 28
390 13
395 14
400 9
405 10
410 14
415 4
420 3
425 19
430 20
435 4
440 5
445 17
450 1
455 2
460 19
465 6
470 6
475 3
480 7
485 7
490 2
495 9
500 11
505 7
510 5
515 3
520 6
525 6
530 5
535 5
540 2
545 7
550 4
555 18
560 2
565 3
570 5
575 17
580 4
585 4
590 5
595 6
600 8
605 3
610 26
615 9
620 1
625 7
630 25
635 20
640 24
645 16
650 5
655 8
660 6
665 11
670 9
675 14
680 12
685 15
690 15
695 5
};
\addlegendentry{5 frames}
\addplot [thin, color3, mark=pentagon*, mark size=0.42, mark options={solid}]
table {%
10 24
20 30
30 14
40 31
50 21
60 12
70 8
80 17
90 13
100 11
110 39
120 24
130 16
140 17
150 10
160 22
170 14
180 6
190 22
200 12
210 8
220 21
230 10
240 23
250 24
260 18
270 16
280 20
290 13
300 15
310 9
320 8
330 1
340 17
350 8
360 13
370 26
380 26
390 28
400 8
410 9
420 13
430 8
440 9
450 4
460 19
470 9
480 11
490 9
500 12
510 4
520 8
530 8
540 4
550 4
560 3
570 21
580 3
590 7
600 5
610 18
620 4
630 29
640 30
650 11
660 15
670 12
680 17
690 11
};
\addlegendentry{10 frames}
\end{axis}

\end{tikzpicture}

